VGX: Large-Scale Sample Generation for Boosting Learning-Based Software Vulnerability Analyses

Accompanying the successes of learning-based defensive software vulnerability analyses is the lack of large and quality sets of labeled vulnerable program samples, which impedes further advancement of those defenses. Existing automated sample generation approaches have shown potentials yet still fall short of practical expectations due to the high noise in the generated samples. This paper proposes VGX, a new technique aimed for large-scale generation of high-quality vulnerability datasets. Given a normal program, VGX identifies the code contexts in which vulnerabilities can be injected, using a customized Transformer featured with a new value-flowbased position encoding and pre-trained against new objectives particularly for learning code structure and context. Then, VGX materializes vulnerability-injection code editing in the identified contexts using patterns of such edits obtained from both historical fixes and human knowledge about real-world vulnerabilities. Compared to four state-of-the-art (SOTA) baselines (pattern-, Transformer-, GNN-, and pattern+Transformer-based), VGX achieved 99.09-890.06% higher F1 and 22.45%-328.47% higher label accuracy. For in-the-wild sample production, VGX generated 150,392 vulnerable samples, from which we randomly chose 10% to assess how much these samples help vulnerability detection, localization, and repair. Our results show SOTA techniques for these three application tasks achieved 19.15-330.80% higher F1, 12.86-19.31% higher top-10 accuracy, and 85.02-99.30% higher top-50 accuracy, respectively, by adding those samples to their original training data. These samples also helped a SOTA vulnerability detector discover 13 more real-world vulnerabilities (CVEs) in critical systems (e.g., Linux kernel) that would be missed by the original model.

==> approach.tex <==
\section{Technical Details of {\tech}}

In this section, we elaborate the design of {\tech} 
%. We separately describe 
by detailing 
its four %technical 
modules shown in Figure~\ref{fig:overview}: \emph{preprocessing}, \emph{semantics-aware contextualization}, \emph{human-knowledge-enhanced edit pattern formation}, and %vulnerability 
\emph{generation}.

\subsection{Preprocessing}\label{ssec:preprocessing}
\vspace{-4pt}
To enable the \emph{semantics-aware contextualization} via the {\tt customized Transformer}, we use 
%to make use of 
\ul{syntactic information} instead of processing code as natural language. Thus, the \emph{preprocessing} begins by converting source code into Abstract Syntax Trees (ASTs) using an AST parser. We employ tree-sitter~\cite{tree-sitter} as the parser following SPT-code~\cite{niu2022spt}. An AST is a tree composed of nodes, each of which has a node type, a set of child nodes, and a value if it is a terminal. 

Since this Transformer %model 
%in \emph{semantics-aware contextualization} 
takes text as %the 
inputs, we linearize the ASTs into text. Following the approach in SPT-Code~\cite{niu2022spt}, we do a pre-order traversal on the AST to get a sequence of node types. However, such sequences may be too long hence %and thus 
negatively impact the performance of the Transformer model~\cite{niu2022spt}. Thus, we only keep the nodes above the expression level. We then concatenate the source code and the linearized AST for each sample with a special token {\tt [SEP]} between them. Therefore, the input of the {customized Transformer} is in the format {\tt Code [SEP] AST} where {\tt Code} is the source code token sequence and {\tt AST} is the linearized AST token sequence. 

To enable the {customized Transformer} to make use of \ul{semantic information}, which can be achieved by position encoding that is explicitly aware of value flow as discussed in $\S$\ref{sec:bkgmotive}, we construct a value flow graph (VFG) for each sample using the tool from GraphCodeBERT~\cite{guo2020graphcodebert}. A VFG is a multi-edge graph $g(V,E)$ with V representing a set of nodes that correspond to the variables in the program, and E representing a set of edges that represent the value flows between different variables. For instance, in an assignment statement such as {\tt c=a+b}, edges would exist from the variable {\tt a} to variable {\tt c} as well as from variable {\tt b} to variable {\tt c}. The arrowed lines in Figure~\ref{fig:illustrate} show parts of the value flows in the motivating example. The VFGs represent the %semantic 
data dependencies between variables, which are widely utilized in code analysis tasks~\cite{guo2020graphcodebert, zhou2019devign, chakraborty2021deep, nong2020preliminary, nong2021evaluating, nong2022open}.



%Since the semantics-aware contextualization step takes value flow graphs (VFGs) and linearized ASTs as (part of) their inputs, in the preprocessing step, we first use an AST parser to convert the source code into ASTs. We use tree-sitter~\cite{tree-sitter} as the AST parser following SPT-code~\cite{niu2022spt}. An AST is a tree containing a set of nodes. Each node has a node type, a set of child nodes, as well as a value if it is a terminal. The ASTs represent the syntactic structures of the source code, allowing the \emph{Customized Transformer} in the \emph{semantics-aware contextualization} step to exploit structural and syntactic information rather than simply processing the code as natural languages.

%as we adapt the source code of SPT-Code~\cite{niu2022spt}, which is based on the AST generated by tree-sitter, to do the AST linearization.

%We use srcML~\cite{collard2013srcml} to generate the ASTs for the pattern mining module as our pattern mining module is based on Getafix~\cite{bader2019getafix} and VulGen~\cite{nongvulgen}, where their pattern mining functionality is adapted for the ASTs generated by srcML. In contrast, for the localization learning module, we use tree-sitter~\cite{tree-sitter} as we adapt the source code of SPT-Code~\cite{niu2022spt}, which is based on the AST generated by tree-sitter, to do the AST linearization.

%While the AST formats of srcML and tree-sitter are different, the ASTs generated by both are in tree structure and contain a set of nodes. Each node has a node type, a set of child nodes, as well as a value if it is a terminal node. The ASTs represent the syntactic structures of the source code, which allow the the pattern mining module to extract and apply edit patterns structurally, and allow the localization learning module to  exploit structural, specifically syntactic, information rather than simply processing the code as natural languages. The ASTs generated by srcML will be fed to the pattern mining module directly for mining vulnerability injection patterns, while the ASTs generated by tree-sitter will be further preprocessed into the localization inputs.

%As we discuss in Section 3, since the localization model is in Transformer structure, it only takes text as the inputs. Thus, to allow the model to process the ASTs, we do AST linearization on the ASTs to convert them into text. We follow the approach in SPT-Code~\cite{niu2022spt} to do the linearization: on the AST, we do a pre-order traversal on the AST to get a sequence of node types. However, since ASTs are in tree structure, sequences obtained by the traversal may be too long for the inputs and impact the performance of the Transformer model. Thus, we also follow the approach in SPT-Code to cut the nodes below the expression level. In this case, we convert the tree-structure ASTs into text. \nong{will show examples later}

%Transformer has been shown to be effective in many code-to-code tasks~\cite{wang2021codet5,fu2022vulrepair, bui2022detect, nong2022generating}. Given the text of the source code, it can generate another fragment of code based on the training tasks. However, it is difficult for it to understand the syntactic information of the code since the source code given is in plain text~\cite{niu2022spt}. Thus, to allow the model to exploit both the plain text of source code and the syntactic structure of the code, for each program, we concatenate the source code and the linearized AST. Between them, we use a special token {\tt [sep]} to separate them. Therefore, the localization input is in the format {\tt Code [sep] L-AST} where {\tt Code} is the source code token sequence of the program and {\tt L-AST} is the linearized AST token sequence. 

%However, ASTs only provide the syntactical structure information of the programs. To make the model understand the code comprehensively, it is also important to exploit the semantic information. Thus, we also leverage the value flow of the programs which provides crucial semantic information of the code~\cite{guo2020graphcodebert}. Given a program, we use a value flow analysis tool from GraphCodeBERT~\cite{guo2020graphcodebert} to extract the value flow graph (VFG). We use this value flow analysis tool because it is integrated with tree-sitter and we can find the respective AST node from the VFG node easily. A VFG is a multi-edge graph $g(V,E)$ where V is a set of nodes representing the variables in the program and E is a set of edges representing the value flows between different variables. For example, in an assignment statement {\tt c=a+b}, there are edges from variable {\tt a} to variable {\tt c} and from variable {\tt b} to variable {\tt c}.\nong{will show a concrete example in a figure later} The VFGs represent the semantic dependencies between variables, which are very helpful for code analysis tasks~\cite{guo2020graphcodebert, zhou2019devign, chakraborty2021deep, nong2020preliminary, nong2021evaluating, nong2022open}.

%Nevertheless, it is difficult to feed the VFGs to the Transformer model as it takes text as the input. We cannot linearize VFGs like ASTs because they are in directed cyclic graph structure while ASTs are in tree structure. GraphCodeBERT~\cite{guo2020graphcodebert} proposes an approach which inputs the sequence of variables in order, and then masks the attention between the variables if they have no value flow path between them. This seems to work but the graph structure information between variables is lost. Therefore, we need an approach that enables the Transformer to utilize the VFG graph structure.

%Based on our literature review, position encoding is proved to be effective and can be tailored to specific tasks~\cite{vaswani2017attention, fu2022vulrepair, peng2021integrating}. Recently, Peng et al.~\cite{peng2021integrating} proposes TPTrans that integrates AST tree paths into Transformer to better represent code. Different from the traditional absolute position encoding~\cite{vaswani2017attention} and relative position encoding~\cite{shaw2018self} which compute the encoding based on the positions (i.e., indexes) of the tokens, it computes the absolute encoding based on the path from the current node to the root node of the AST and computes the relative encoding based on the path from the source node to the target node on the AST. The sequence of nodes on the path is fed into a Gated Recurrent Unit (GRU) model to generate the encoding. This specific position encoding is shown to be more effective on analyzing code~\cite{peng2021integrating}.

We develop our value-flow-based position encoding following the traditional position encoding %which is 
based on the indexes of tokens, by which 
%In the original 
absolute position encoding %, the encoding 
is calculated based on the absolute position (i.e., index) of a given token. In our approach, we calculate the absolute position encoding of a variable based on its respective \ul{absolute VFG sub-graph}. To obtain this %the absolute VFG 
sub-graph, 
we backtrack the nodes from the current node on the extracted VFG until no new nodes can be found. 
%included in the sub-graph. 
For instance, in Figure~\ref{fig:illustrate}, the token {\tt password} at Line 10 has the value flow marked as red, and thus its absolute VFG sub-graph consisting of itself and the node of token {\tt password} at Line 1.

Similarly to the original relative position encoding, which computes the encoding based on the distance between a pair of tokens, our approach calculates the relative position encoding for a pair of variables based on their respective \ul{relative VFG sub-graph}. To obtain 
%the relative VFG 
this 
sub-graph, we backtrack the nodes from the source node on the extracted VFG until we reach the target variable. Only the nodes on the paths from the source variable to the target variable are included in the sub-graph. For example, in Figure~\ref{fig:illustrate}, the pair of variables {\tt buf} at Line 6 and {\tt BUFSIZE} at Line 3 have their relative VFG sub-graph consist of the nodes of tokens {\tt buf} at Line 6, {\tt buf} at Line 4, {\tt buf} at Line 3, and {\tt BUFSIZE} at Line 3.

In this case, given a variable or a pair of variables in a program,
we can create a respective absolute and relative VFG subgraph. The subgraphs can be further embedded by a gated graph neural network (GGNN) model, and the resulting embeddings are used for the position encoding. We will provide further details on this process in $\S$\ref{ssec:sac}.


%we extract a set of relative VFG sub-graphs and a set of absolute VFG sub-graphs. The sets of sub-graphs will be fed into the self-attention blocks of the Transformer model for VFG-based position encoding.

\subsection{Semantics-Aware Contextualization}\label{ssec:sac}
\vspace{-4pt}
In this step, we train a {\tt customized Transformer} in order to achieve \emph{semantics-aware contextualization}. Given a normal program with the \emph{Code+AST} input, we expect the model to output a code fragment that can be manipulated to introduce a vulnerability, based on the semantics and context of the code. To that end, the {customized Transformer} leverages \emph{value-flow-based position encoding, pre-training,} and \emph{fine-tuning} with data augmentation. We separately describe these in the following subsections. 

%To achieve this, we pass the \emph{Code+AST} inputs from the \emph{preprocessing} step into an \emph{input embedding} layer to convert the tokens into vectors. These vectors are then fed into the Transformer model that utilizes \emph{value-flow-based position encoding}. The outputs of the model are expected to be the identified statements that can be exploited to introduce vulnerabilities.

%To improve the model's ability in code understanding and localization, we first pre-train the model on a large code corpus against 3 existing general-purpose programming-language-oriented objectives and 2 new code-localization-specific objectives. Then, we fine-tune the model on an existing dataset of vulnerability-introducing code locations augmented by their refactored versions. We separately discuss the details in the following subsections.

%before fine-tuning for vulnerability injection localization to improve the model understanding of code. To deal with the issue that there is a lack of vulnerability fixing data for training, we also do data augmentation on the training data. We separately discuss the three mechanisms in the following subsections.

%Then, they are fed into an encoder stack and then a decoder stack to output the localization results. The encoder stack and decoder stack are based on standard Transformer model~\cite{vaswani2017attention}. We only specify the self-attention block which is one of the core components of the model. Besides, we pre-train the model before fine-tuning for vulnerability injection localization to improve the model understanding of code. To deal with the issue that there is a lack of vulnerability fixing data for training, we also do data augmentation on the training data. We separately discuss the three mechanisms in the following subsections.

\subsubsection{Value-flow-based Position Encoding}
In the encoder of Transformer, the self-attention block uses \emph{key} and \emph{value} pairs to \emph{query} the attention which can be computed as follows:
\begin{equation}
    Attention(Q,K,V)=softmax(\frac{QK^T}{\sqrt{d}})V
\end{equation}
where $Q,K,V$ are the hidden representations of \emph{query, key,} and \emph{value} from the previous layer respectively and $d$ is the dimension of the hidden representations. To better explain the attention, we can expand the equation as follows:
\begin{equation}
    z_i=\sum^{n}_{j=1}\frac{exp(a_{ij})}{\sum^{n}_{j'=1}exp(a_{ij'})}(x_jW^V)
\end{equation}
where $z_i$ is the output hidden representation for the $i$-th token, $a_{ij}$ is the attention between the $i$-th and $j$-th tokens, $x_j$ is the %$j$-th 
hidden representation of the $j$-th token from the previous layer, and $W^V$ is the weight matrix of \emph{value}. For $a_{ij}$, we can further expand it as follows:
\begin{equation}
    a_{ij}=\frac{1}{\sqrt{2d}}(x_iW^Q)(x_jW^K)^T
\end{equation}
where $W^Q$ and $W^K$ are the weight matrices of \emph{query} and \emph{key}, respectively. 

To improve the effectiveness of the attention blocks, previous works add \emph{absolute position encoding}~\cite{vaswani2017attention} and \emph{relative position encoding}~\cite{shaw2018self} to %the 
each attention block. 
Specifically, the attention block with the two kinds of encoding is as follows:

\begin{equation}
    z_i=\sum^{n}_{j=1}\frac{exp(a_{ij})}{\sum^{n}_{j'=1}exp(a_{ij'})}(x_jW^V+r^{V}_{ij})
\end{equation}
\begin{equation}
    a_{ij}=\frac{1}{\sqrt{2d}}(x_iW^Q)(x_jW^K+r^{K}_{ij})^T+\frac{1}{\sqrt{2d}}(a^Q_i)(a^K_j)^T
\end{equation}
where $r^{V}_{ij}$, $r^{K}_{ij}$ are the relative position encodings for \emph{value} and \emph{key} respectively, and $a^Q_i$ and $a^K_j$ are the absolute position encodings for \emph{query} and \emph{key} respectively. 

To take the advantages of the traditional position encoding, \textit{we keep the two kinds of encoding described above in our model}. We follow the original algorithm to calculate the absolute position encoding~\cite{vaswani2017attention} and the relative position encoding~\cite{shaw2018self}. Specifically, $a^Q_i=p_iA^Q$ and $a_j^K=p_jA^K$ where $p_i$ and $p_j$ are the sine and cosine functions of the positions $i$ and $j$, respectively. $A^Q$ and $A^K$ are the weight matrices of \emph{query} and \emph{key}~\cite{vaswani2017attention}, respectively. 
$r_{ij}^V=(i-j)R^V$ and $r_{ij}^K=(i-j)R^K$ where $R^V$ and $R^K$ are the weight matrices for relative position encoding~\cite{shaw2018self}.

However, the traditional position encoding is solely based on the positions (indexes) of tokens hence \textit{lacks semantic understanding of code}. For example, a variable is defined at one line but used many lines after. 
%many lines of code. 
In this case, the distance $(i-j)$ used by the relative position encoding may be too large, %"far away", 
although the two variable tokens may share a direct definition-use relationship and have a close 
semantic (i.e., value-flow) 
distance. 
To address this limitation, we also utilize the VFG sub-graphs obtained during preprocessing %, module 
to \textit{incorporate semantic information into the position encoding}.

Specifically, the attention block with our value-flow-based position encoding added is as follows:
\begin{equation}
    z_i=\sum^{n}_{j=1}\frac{exp(a_{ij})}{\sum^{n}_{j'=1}exp(a_{ij'})}(x_jW^V+r^{V}_{ij}+r^{V_{VFG}}_{ij})
\end{equation}

\begin{multline}
    a_{ij}=\frac{1}{\sqrt{2d}}(x_iW^Q)(x_jW^K+r^{K}_{ij}+r^{K_{VFG}}_{ij})^T \\
    +\frac{1}{\sqrt{2d}}(a^Q_i)(a^K_j)^T+\frac{1}{\sqrt{2d}}(a_i^{Q_{VFG}})(a_j^{K_{VFG}})^T
\end{multline}
where $r^{V_{VFG}}_{ij}$, $r^{K_{VFG}}_{ij}$, $a_i^{Q_{VFG}}$, and $a_j^{K_{VFG}}$ are the graph encoding of the respective sub-graphs. 

To compute the encoding of a given VFG sub-graph $g(V,E)$, we first use a pre-trained FastText~\cite{bojanowski2016enriching} model for C language to convert the variable name in each node into an embedding. Then, for each node embedding $x_v$, we use a GGNN model to perform message passing aggregation and update the node embedding as follows:
\begin{equation}
    x'_v=GRU(x_v, \sum_{(u,v)\in E}g(x_u))
\end{equation}
where GRU is the gated recurrent function, $g(.)$ is the function that assimilates the neighbor nodes' embedding, and $x_u$ is the neighbor node of $x_v$. After the message passing aggregation, we sum up the nodes in the graph to get the VFG sub-graph embedding:
\begin{equation}
    x_g=\sum_{v \in V} x'_v
\end{equation}

Finally, the graph embedding is multiplied with a weight matrix to get the \ul{value-flow-based position encoding}:

\begin{equation}
    r_{ij}^{V_{VFG}}=x_gR^V_{VFG}
\end{equation}
\begin{equation}
    r_{ij}^{K_{VFG}}=x_gR^K_{VFG}
\end{equation}
\begin{equation}
    a_{i}^{Q_{VFG}}=x_gA^V_{VFG}
\end{equation}
\begin{equation}
    a_{j}^{K_{VFG}}=x_gA^K_{VFG}
\end{equation}

Note that not all code tokens are variables. Thus, we only compute the value-flow-based position encoding when the token or both the tokens in the pair are variables. Otherwise, the value-flow-based position encoding is zero.

\subsubsection{Pre-Training}
%Pre-training has been demonstrated to be an effective technique for natural language understanding and programming language modeling~\cite{devlin2018bert, feng2020codebert, wang2021codet5, niu2022spt}. It allows us to train a model effectively even when working with limited amounts of training data, which is the case in our work. Therefore, 

To gain the awareness of code semantics, we performed pre-training before fine-tuning the model for \emph{semantics-aware contextualization}. We use three existing general-purpose programming language-oriented objectives 
%(\textit{CodeT5 objectives}) 
and introduce two \ul{new code %localization
contextualization-specific objectives} ({\tt CAP} and {\tt ISP}) for pre-training.

\textbf{CodeT5 Objectives.} %We aim to enable the model to comprehend code effectively for code-to-code tasks. Therefore, 
We utilize three pre-training objectives from CodeT5~\cite{wang2021codet5} to %comprehend code 
learn general code comprehension 
effectively for code-to-code transformation. The first objective is {\tt mask span prediction (MSP)}, where we randomly mask 15\% of the source code tokens in an input that contains both source code and AST, with each mask having a span length uniformly ranging from 1 to 5 tokens. We train the model to recover the masked tokens based on the context. The second objective is {\tt identifier tagging (IT)}, where the model is trained to predict whether each source code token is an identifier. The third objective is {\tt masked identifier prediction (MIP)}, where we mask all the identifiers in the source code, and the model is trained to recover the identifiers based on the code semantics. We follow the pre-training approach of CodeT5, and feed the three pre-training objectives alternatively during training with an equal probability.

\textbf{Code-AST Prediction (CAP).} Since our model takes source code and ASTs as input, similar to SPT-Code~\cite{niu2022spt}, we adopt their approach and pre-train our model with the Code-AST Prediction (CAP) objective. In this objective, we randomly assign the correct AST to the corresponding source code in 50\% of the pre-training samples, while in the other 50\%, we randomly assign an incorrect AST. Our model is then trained to predict whether the assigned AST corresponds to the input source code.

\textbf{Irrelevant Statement Prediction (ISP).} In this objective, we randomly insert a statement from another sample into a random location of the current sample for each pre-training sample. The inserted statement is not semantically related to the original sample and the model is trained to identify and output the irrelevant statement. We adopt this pre-training objective because it resembles our vulnerability injection localization objective. 
%Since vulnerabilities are security weaknesses in programs, statements that can introduce vulnerabilities are usually not relevant to the main functionalities of the programs. 
Since \textit{vulnerabilities are context-sensitive based on 
%and the sensitivity is rooted in 
code semantics, learning to differentiate (semantically) irrelevant statements (from relevant ones) intuitively helps identify the right code context that is (semantically) relevant to the vulnerabilities to be injected}. 
%Thus, such a pre-training objective is effective to enhance the \emph{semantics-aware contextualization}.

We conduct pre-training in the following order: first against CAP, then the three CodeT5 objectives, and finally ISP, as justified by the inter-dependencies among these objectives. 
%During CAP pre-training, we only pre-train the encoder. For CodeT5 objectives, we pre-train both the encoder and decoder on MSP and MIP, while on IT, we only pre-train the encoder. For ISP, we pre-train both the encoder and decoder. 
Also, for CAP and one of the CodeT5 objectives (IT), the pre-training is done on the encoder only, while for all the other objectives (ISP, MSP, MIP) we pre-train both the encoder and decoder. 
These decisions are justified by the nature of the Transformer architecture. 

\subsubsection{Fine-Tuning}\label{ssec:ft}
After the pre-training, we fine-tune the model to locate code fragments that can be edited %manipulated 
to introduce vulnerabilities, using the vulnerability-introducing code locations retrieved from the existing vulnerability fixes.
To address the lack of fine-tuning data, we perform \ul{data augmentation} through code refactoring on the fine-tuning samples. Following the approach in \cite{nong2022generating}, we apply three types of \textit{semantics-preserving refactoring}: (1) reverse the condition in an {\tt if}-statement and swap the code in the {\tt if} and {\tt else} blocks; (2) convert a {\tt for} loop into an equivalent {\tt while} loop; and (3) insert unrelated junk code generated by SaBabi~\cite{sestili2018towards} to the code. We apply these transformations combinatorially on each original sample, leading to substantially more fine-tuning samples. 



\subsection{Edit Pattern Formation}\label{ssec:hkeepf}
\vspace{-4pt}
This section describes the process of {\tech} on learning to materialize the code editing for realizing vulnerability injection from existing such concrete edits, including \emph{pattern extraction, pattern filtering and ranking, pattern refinement,} and \emph{pattern diversification}.
%in the following subsections. 
%
%In this step, we first \emph{extract} the vulnerability-introducing code edit patterns from the \emph{existing vulnerability fixes}, followed by \emph{pattern filtering/ranking} to get relatively appropriate patterns. Then, we \emph{refine} the patterns by \emph{manually deriving patterns} based on \emph{human knowledge discovery}, such as common patterns manually observed in vulnerability documentation. Finally, we \emph{diversify} the patterns using the \emph{manually derived pattern mutation rules} which are also based on \emph{human knowledge discovery}, such as rules for adding, deleting, or modifying code elements in the patterns to create new and varied patterns.

\subsubsection{Pattern Extraction}
We first parse the source code into ASTs like the one for \emph{semantics-aware contextualization} but with a different AST parser srcML~\cite{collard2013srcml}, as it better supports edit pattern extraction and application~\cite{bader2019getafix,nongvulgen}. Then, we follow the approach in Getafix~\cite{bader2019getafix} to \ul{extract the edit patterns} by anti-unification. Because of the space limit, we refer this part to the original Getafix paper~\cite{bader2019getafix}. After the pattern extraction, we get many edit patterns that range from very general (i.e., the patterns that can match and apply on many different code samples) to very specific (i.e., the patterns that can only match and apply on a few code samples)~\cite{bader2019getafix}. For example, %formulas 14-16 
Formulas~\ref{pattern1}--\ref{pattern3}
show three edit patterns from specific to general. %In formula 14, 
In Formula~\ref{pattern1},
all the identifiers (i.e., {\tt buf} and {\tt size}) and literals (i.e., {\tt 1} and {\tt 0}) are specified, while %in formula 15, 
in Formula~\ref{pattern2}, 
only the literals ({\tt 1} and {\tt 0}) are specified. %and in formula 16,
In Formula~\ref{pattern3},
all the identifiers and literals are placeholders (i.e., {\tt h0, h1, h2}, and {\tt h3}) where they can match any identifiers and literals. 




%It first takes the pairs of the parsed ASTs from the preprocessing module. In a pair of ASTs, one is the vulnerable version of the program, and the other is the respective non-vulnerable fixed version. Since the non-vulnerable version is the fixed one of the vulnerable program, it is probably that most of the code is the same and only a few statements are changed. Thus, we only want to extract the changed parts of the code. We use a syntax-aware AST differencing tool GumTree~\cite{falleri2014fine} to do this because it supports processing the ASTs from srcML. The extracted concrete edits are pairs of AST subtrees that are changed in the programs. In this case, the concrete edits can match different programs even if the non-changed contexts are different. Therefore, they are good base for vulnerability injection patterns.

%However, the concrete edits are "concrete" because all the nodes in the pairs of subtrees are directly from the training examples. They cannot match a subtree if any of the nodes in the subtree are different from the ones in the concrete edits. Thus, we hope that the edits can be more general and some nodes in the subtrees can match different nodes. In this case, we use the anti-unification algorithm from Getafix~\cite{bader2019getafix} to merge different concrete edits so that a merged edit is generalized for all the examples used to get it. For example, to inject a buffer overflow vulnerability, two different concrete edits may be like:
\begin{equation}\label{pattern1}
     buf[size-1]=0; \Longrightarrow buf[size]=0;
\end{equation}
% \begin{equation}
%      buf2[size2-1]='\textbackslash 0'; \Longrightarrow buf2[size2]='\textbackslash 0';
% \end{equation} 
% as the buffer name and buffer size may be different in different examples. After merging with the anti-unification algorithm, the edit is 
\begin{equation}\label{pattern2}
    h0[h1-1]=0; \Longrightarrow h0[h1]=0;
\end{equation}
\begin{equation}\label{pattern3}
    h0[h1-h2]=h3; \Longrightarrow h0[h1]=h3;
\end{equation}
% where {\tt h0} and {\tt h1} are \emph{holes} can match any variable name and the size respectively. The merged edits are named abstract edits, and the abstract edits can be further merged with other concrete or abstract edits to get more general abstract edits.

% Nevertheless, the anti-unification algorithm only merges two edits at a time. There are many concrete edits to be merged. Thus, to find the most appropriate edits to merge, we further follow Getafix~\cite{bader2019getafix} to use the hierarchical clustering to merge the edits to get a set of edit patterns. The edit patterns can range from very specific to very general~\cite{bader2019getafix}.  
% Since the anti-unification and the hierarchical clustering algorithms are complex, we refer this part to the original Getafix paper~\cite{bader2019getafix}.

\begin{table}[htbp]
  \centering
  \caption{\modify{Manually Defined Patterns}}
    \scalebox{0.75}{
        \begin{tabular}{|p{14em}|p{15em}|}
        \hline
        Manually derived pattern & Justification \\
        \hline
        *mutex*(h0); => EMPTY & 
        “Race Condition” mostly happens with a lack of mutex related statements, but there are many  mutex related function~\cite{race-condition}. Thus, once the located statement involve “mutex”, we delete it. \\
        \hline
        *TCHECK*(h0); => EMPTY & There are many samples in the train- \\
        *assert*(h0); => EMPTY & ing set deleting statements involving "TCHECK" and "assert", but they usually use different function names\cite{tcheck}. Thus, once located statement involve “TCHECK” or “assert”, we delete it. \\ 
        \hline
        *free*(h0); => EMPTY & "Memory Leak" mostly happens with   \\
        *Free*(h0); => EMPTY & not releasing assigned memory. \\
        *destruct*(h0); => EMPTY &  However, there may be many differ-  \\
        *destroy*(h0); => EMPTY & ent functions for releasing the mem-  \\
        *unref*(h0); => EMPTY & ory~\cite{memleak}. Thus, once the the located   \\
        *clear*(h0); => EMPTY & statement involve memory release related functions, we delete it. \\
        \hline
        static h0 h1 = h2; => h0 h1 = h2; & "Type Error" usually happens with  \\
        unsigned h0; => h0; & not using static, unsigned, large-size  \\
        int64\_t h0; => int h0; & types, but the current patterns specify too many details like identifier names or assigned values in the patterns~\cite{typeerr}. Thus, we make these details holes so that they are more general. \\
        \hline
        memset(h0); => EMPTY & "Use of Uninitialized Variables" usu-\\
        h0 = *ERR*; => EMPTY & ally happens with not initializing de- \\
        h0 = *NONE* => EMPTY & clared variables, but current  \\
        h0 = 0; => EMPTY & patterns specify too many details like \\
        h0 = NULL; => EMPTY &  identifier names and values in the \\
        *buf* = h0; => EMPTY &  patterns~\cite{uninit}. Thus, we make these details holes and use regular expression to represent the common initialized value, so that they are more general. \\
         \hline
        h0 = kcalloc(hole1, hole2, hole3);  & "Memory Allocation Vulnerability"  \\
                    \hspace{0.5em} => h0 = kzalloc(h1*h2, h3); & usually happens when using unsafe memory allocation functions, but \\
        h0 = calloc(hole0, hole1);  &  current patterns specify too many de- \\
                   \hspace{0.5em} => h0 = malloc(h1*h2); & tails like identifier names and values in the patterns~\cite{allocerr}. Thus, we make them holes to make the patterns more general. \\
        \hline
        \end{tabular}
    }
    \label{tab:derived-patterns}
\end{table}

\begin{table*}[htbp]
  \centering
  \caption{\modify{Pattern Mutation Rules}}
    \scalebox{0.75}{
    \begin{tabular}{|p{40em}|p{20em}|}
    \hline
    Pattern Mutation Rule & Justification \\
    \hline
    \textbf{Function call return value assignment mutation:} & Some function calls like strncpy may return some  \\
    function\_call\_name(parameters); =>new\_function\_call\_name(new\_parameters); & values but the return values do not always assign  \\
    \hspace{5em}$\Updownarrow$ & to a variable. Mutating such patterns so that they  \\
     h0=function\_call\_name(parameters); => h0=new\_function\_call\_name(new\_parameters);& have or remove the return value assignments increases the generalizability of the pattern set.\\
    \hline
    \textbf{Returned error code mutation:} & The typical safety issue checks do some check  \\
    if(condition) {return NULL/0/-1;} => EMPTY & in an if statement condition and then return  \\
    \hspace{5em}$\Updownarrow$ & an error code when found the issue. However,  \\
    if(condition) {return -EINVAL/EBADFD/ENOTSOCK/EPERM/ENODEV/ENOMEM;} => EMPTY & there are many possible returned error codes. We  \\
    \hspace{5em}$\Updownarrow$& mutate these returned error codes to make the  \\
    if(condition) {return;}=> EMPTY & patterns more general. \\
    \hline
    \textbf{Safety check condition generalization mutation:} & In our automatic pattern mining, the mined safety  \\
    if(specific\_condition) {return error\_code;} => EMPTY & checks if statements may be too specific in the \\
    \hspace{5em}$\Downarrow$& condition. However, if an if statement only has  \\
    if(hole) {return error\_code;}=> EMPTY & one return statement, it is very likely that it is a safety check if statement. Thus, we remove the specific conditions in these if statements and use a hole to make the patterns more general. \\
    \hline
    \textbf{Safety check exit statement mutation:} & When the safety checks if statements find issues,  \\
    if(condition) {return error\_code;}=> EMPTY & they may not always exit the function using  \\
    \hspace{5em}$\Updownarrow$& a return statement. If the safety check is in a \\
    if(condition) {break;} => EMPTY & for/while/switch block, it may use a break or  \\
    \hspace{5em}$\Updownarrow$& continue statement to exit. Thus, we mutate the  \\
    if(condition) {continue;}=> EMPTY & exit statement to make the patterns more general. \\
    \hline
    \end{tabular}}
  \label{tab:mutation}
\end{table*}
\subsubsection{Pattern Filtering/Ranking}
To obtain the appropriate edit patterns for introducing vulnerabilities, we establish rules to filter and rank the extracted patterns. \ul{First},  compute three scores for each of the %remaining 
extracted 
edit patterns: %to rank them:
%
%Firstly, we \textbf{filter out the edit patterns without specified identifier names} since they are too general and lack semantic meaning that is often reflected in the identifier names. Subsequently, we compute three scores for each of the remaining edit patterns to rank them:
%With the anti-unification and the hierarchical clustering, we get too many edit patterns. Thus, {\tech} needs to appropriately select a pattern that can successfully inject a vulnerability given a program. In this case, we set rules to filter and rank the extract patterns. We first remove the edit patterns with no specified identifiers because they are too general and have no sense to the code semantic, which are often revealed in the identifier names. Then, we compute three scores for each of the remaining edit patterns to rank them: 
\begin{enumerate}
    \item \textbf{Prevalence score ($s_{preval}$)}: Assuming we know the correct location to inject the vulnerability, we apply the pattern to all the training samples, and the prevalence score is the number of samples that can be injected the vulnerabilities successfully.
    \item \textbf{Specialization score ($s_{spec}$)}: We compute the average number of AST subtrees in a program that the pattern can match. The reciprocal of the average number is then used as the specialization score.
    \item \textbf{Identifier score ($s_{ident}$)}: The identifier score is the number of specified identifier names in the patterns.
\end{enumerate}

Then, we compute the final ranking score by multiply the three scores:
\begin{equation}\label{rankingeq}
    s_{rank}=s_{preval}\times s_{spec}\times s_{ident} 
\end{equation}

\ul{Second}, we rank the edit patterns by %the ranking 
these scores in a reversed order. The higher ranking score, the more likely that the pattern can help successfully inject vulnerabilities. \ul{Third}, we only keep the first 300 edit patterns to filter out those %the patterns 
that are not likely to help inject vulnerabilities successfully.

\subsubsection{Pattern Refinement}
\modify{We then refine the extracted patterns because some of them are too general or too specific~\cite{bader2019getafix}. We applied the 300 filtered patterns to the vulnerability-introducing training samples. As a result, we encountered \textit{false positives}, where the pattern was applied but the generated sample was not actually vulnerable, as well as \textit{false negatives}, where none of the 300 patterns could be applied.}

\modify{For the false positives, we consider that the patterns applied on them are \ul{too general}. 
We then removed the patterns against which more than half of the applications are false positives. 
In total, we removed 21 patterns in this manner.}


\modify{For the false negatives, we consider that the corrresponding patterns are \ul{too specific}. Thus, we need to \ul{manually define new patterns} that are necessarily more general. 
To do so, we examined the commit messages associated with false negatives and identified the corresponding CWE IDs for the corresponding sample using the CWE report~\cite{cwereport}.}

\modify{Then, we read the CWE document and check the synthetic examples used to describe the CWE ID. We also go to the CVE/NVD database~\cite{nvd} to check other real-world vulnerability samples with the same CWE ID. Based on the false negative, the synthetic example, and other real-world samples, we compose/envision several possible patterns that can cover them. Then, we go back to the existing pattern set and find patterns close to the envisioned ones. We finally modify these patterns into the envisoned patterns with the use of regular expression (regex). These modified patterns are the 20 manually defined new patterns described in Table~\ref{tab:derived-patterns}. For example, we notice that there are many false negatives happening on project-defined functions for freeing/releasing pointers (e.g., Figure~\ref{fig:case-re}). It is difficult for the patterns to cover all these statements. Thus, we manually define patterns with regular expressions so that once the function-call name involves pointer freeing keywords like "free", "release", etc., we can match and apply the patterns.}



% After pattern filtering/ranking, we notice that some patterns are still so general that they match the AST subtrees that cannot be injected vulnerabilities. Some other patterns are too specific to match the code that can be injected vulnerabilities. Thus, we applied manual \emph{pattern refinement} to the 300 edit patterns %and first remove 
% hence removed 21 too-general ones. 
% To make the too-specific patterns more general, we \emph{manually define patterns} that enable regex %regular expression 
% on the identifier names. %Table~\ref{tab:derived-patterns} in Appendix~\ref{sec:manualpatterns} %A shows the patterns we derive and the respective justifications for them. 
% We finally added 20 %modified 
% edit patterns, %and the refined edit pattern set has 299 patterns. 
% ending up with 299 refined patterns. 
% The refinement process, the process of \ul{human knowledge discovery} by which the
% 20 patterns were defined, and the resulting patterns (Table~\ref{tab:derived-patterns})
% and their justifications 
% are all detailed in Appendix~\ref{sec:manualpatterns}.


\subsubsection{Pattern Diversification}
Since manual refinement is costly, we are not able to derive many new patterns. %samples. 
Some remaining patterns are still too specific in syntactic structure. Thus, we further derived a set of pattern mutation rules to make the edit patterns 
sufficiently
general. \modify{We carefully check the traditional mutation operators for C language~\cite{agrawal1989design}. We select those without changing the code functionality significantly and finally derive four types of pattern mutation rules: \textit{function call return value assignment mutation}, \textit{returned error code mutation}, \textit{safety check condition generalization mutation}, and \textit{safety check exist statement mutation}. Table~\ref{tab:mutation} shows the pattern mutation rules we derived and the respective justifications for them. $\Updownarrow$ means the mutation is bidirectional, while $\Downarrow$ means the mutation is unidirectional.} After the mutation, we get a total of 604 high-quality \emph{vulnerability-injection code edit patterns}.




\subsection{Vulnerability Production}\label{ssec:production}
\vspace{-4pt}
With the trained \emph{contextualization} model and the \emph{vulnerability-injection code edit patterns}, {\tech} is ready to produce vulnerability data. Given a normal program, we again preprocess it like we do in the learning/training phase. Next, the %trained 
\emph{contextualization} model %locates
identifies 
a code fragment (as the context) for vulnerability injection. Then, {\tech} applies the most suitable pattern to the %located code fragment. 
identified context. 
To do so, we rank the patterns in the final set of \emph{vulnerability-injection code edit patterns} %with the ranking score in equation 17, 
by the score computed in Equation~\ref{rankingeq} 
and apply the first 
pattern in the set that can match the %located code fragment. %in the set. 
context. 
Note that {\tech} only injects the vulnerability when one of the patterns matches the context. %located code. 
If none of the patterns matches, {\tech} discards the sample to reduce false positives. Otherwise, the program with the pattern applied is expected to be vulnerable. 







==> intro.tex <==
\section{Introduction}
Software vulnerabilities are the major threats to cybersecurity. They can be exploited and thus cause  software crashing, data tampering, and sensitive information leakage~\cite{realvul2020}. In response, many researchers and developers have designed various kinds of technical approaches to defend against software vulnerabilities~\cite{fu2021flowdist, wen22fsetool, nong2021evaluating, yu2020study}. Among many kinds of vulnerability analysis approaches, deep learning (DL) based approaches are the most momentous ones~\cite{wu2022vulcnn, zou2022mvulpreter, zhou2022vulnerability, le2022use, hin2022linevd}. They achieve great success and are reported surpassing other kinds of vulnerability analysis approaches.

However, these great successes are usually evaluated on synthetic programs. When we evaluate the techniques on real-world scenarios (i.e., detecting vulnerabilities in large and complex real-world software), they perform much worse than what they report~\cite{zhou2019devign,chakraborty2021deep}. Thus, we need large and complex vulnerability datasets which represent real-world vulnerability scenarios to train powerful DL-based models. However, the existing complex vulnerability datasets collected from real-world projects \cite{booth2013national,fan2020ac,wang2021patchdb,bhandari2021cvefixes} are not sizable enough. Therefore, an intuitive solution is to automatically generate such large and complex vulnerability datasets~\cite{nong2022generating}. 

A few vulnerability data generation approaches exist~\cite{bader2019getafix,zenong281412,patra2021semantic,nong2022generating,zhang2021framework,nongvulgen}, but they still face critical challenges due to the following limitations:
\begin{enumerate}
    \item \textbf{The vulnerability generation patterns are ambiguous.} Some existing works use pattern mining/application approaches to generate vulnerabilities~\cite{bader2019getafix,zenong281412}, but they suffer from ambiguity because the patterns are syntax-based and are not aware of the code semantics, thus the patterns are either too generic or too specific to be applicable.
    \item \textbf{The vulnerability generation approaches also suffer data-shortage problem by themselves.} Some works use DL models that are aware of code semantics to generate vulnerability data~\cite{nong2022generating,nongvulgen}, but since DL models need large-scale data to train them well and there is a lack of vulnerability data, they also suffer the data-shortage problem.
    \item \textbf{The generated vulnerability samples are monotonous.} Some other existing works build high-quality rules to generate vulnerability samples~\cite{zhang2021framework,zenong281412}, but the rules are monotonous because they are completely manually derived, making the generated samples only cover one or a few vulnerability types.
    \item \textbf{The generated vulnerability data has much noise.} Most of the existing vulnerability generation approaches cannot guarantee the precision of the generated data, thus they are not useful for training better vulnerability analysis models.
    
\end{enumerate}
 
To tackle these challenges, we propose {\tech}, a novel automatic vulnerability sample generation approach that aims at generating diverse, complex, and precise vulnerability data for data-driven vulnerability analysis techniques to learn. Similar to VulGen~\cite{nongvulgen}, {\tech} learns to inject vulnerabilities from the reversed pairs of vulnerable and respective fixed (normal) programs. Then, given a large number of normal programs, {\tech} generates large-scale vulnerable programs.
We follow VulGen~\cite{nongvulgen} to decouple where to inject and how to inject because this approach is proved to be effective.
 However, our approach comprehensively overcomes the limitation of VulGen as VulGen is not semantics-aware and is subject to the overfitting to the seed samples, making it generate samples of undesirable quality (level of noise is high).

We fine-tune a pre-trained Transformer~\cite{vaswani2017attention} to do vulnerability injection localization. We use a specific designed pattern mining and application model to inject vulnerabilities to the located statements. Our vulnerability injection localization Transformer leverages structural information of the code, value flow-based attention mechanism, localization-specified pre-training design, and data augmentation. These makes the vulnerability data generation semantics- and context-aware. It effectively disambiguate the generic patterns and complementary to the merits of code pattern based injection editing. The pattern mining and application model leverages human-knowledge-based edit pattern diversification to enable generating samples beyond the seeds, overcoming potential overfitting. This is essential because we cannot gather seed samples that cover all the existing vulnerability knowledge like those reflected in CWE descriptions and CVE cases. 

We evaluate {\tech} on a real-world vulnerability dataset containing 7764 pairs of normal functions and respective vulnerable ones for training and testing. {\tech} achieves 59.46\% precision, 22.71\% recall, and 32.87\% F1 where a true positive sample is the one exactly matches the ground-truth vulnerable sample. By manual inspecting the generated samples, the success rate (percentage of generated samples that are indeed vulnerable) is 78.55\% which is comparable to the existing vulnerability datasets where their label accuracy is up to 80\%~\cite{croft2023data}. Compared with other vulnerability generation approaches, {\tech} outperforms them by 239.77\%-1173.23\%, 44.28\%-780.23\%, 99.09\%-890.06\%, and 16.70\%-294.92\% in terms of precision, recall, F1, and success rate respectively. 

We also evaluate the usefulness of {\tech} on large-scale vulnerability sample generation. We collect the latest source code of 238 projects that are involved in the CVE/NVD database~\cite{nvd} and extract 738,453 normal samples at function level. {\tech} successfully generates 150,392 samples with success rate 78.13\% in 50 hours 48 minutes. By augmenting the training sets of the existing downstream vulnerability analysis tools, we improve (1) function-level vulnerability detectors by 9.67\%-330.80\% in terms of F1; (2) line-level vulnerability localization tools by 12.86\%-13.31\% in terms of top-50 accuracy; and (3) vulnerability repair tools by 85.02\-99.30\% in terms of top-50 accuracy. With our augmented datasets, the improved vulnerability detection models detect x more latest vulnerabilities reported on CVE/NVD~\cite{nvd} database, indicating the usefulness of {\tech}. 

Overall, our work makes the following main contributions:
\begin{itemize}
    \item We propose {\tech}, a vulnerability generation approach which leverages specific designed pre-training, attention mechanism, data augmentation, and human knowledge to overcomes the limitations of existing vulnerability generation approaches.
    \item We evaluate {\tech} and show the promising effectiveness of {\tech} in generating vulnerability data.
    \item We apply {\tech} on real-world normal programs and successfully generate a large-size vulnerability dataset with 150,392 vulnerable samples. The generated dataset is complex, diverse, and with low noise.
    \item We use the generated data to augment the existing training datasets for vulnerability detection, vulnerability localization, and vulnerability repair. The augmented training datasets successfully improve all the models, and the vulnerability detection models are able to find the latest vulnerabilities after the improvement.
\end{itemize}



==> overview-cai.tex <==
% root: paper.tex
\section{Overview of {\tech} Design}\label{sec:overview}

\begin{figure*}[tp]
\centering
\vspace{-0pt}
%\includegraphics[width=0.9\linewidth]{figures/overview-cai-grey.pdf}
%\includegraphics[width=0.9\linewidth]{figures/overview-cai.pdf}
%\includegraphics[width=0.9\linewidth]{figures/overview-cai-grey-final.pdf}
%\includegraphics[width=0.9\linewidth]{figures/overview-cai-grey-final.pdf}
\includegraphics[width=0.8\linewidth]{figures/overview-cai-finalized.pdf}
\vspace{-10pt}
\caption{Design overview of the {\tech} approach, highlighting its two main phases: \textit{learning/training} and \textit{production}.}
\label{fig:overview}
\vspace{-10pt}
\end{figure*}

%As noted earlier, 
The overarching \textbf{design goal} of {\tech} is two-fold:
(1) \textit{large-scale}---being able to generate a massive number of samples to meet the thirsty need of training powerful defensive models, which requires the ability to inject vulnerabilities to 
normal code in the wild when following the injection-based methodology, and 
(2) \textit{high-quality}---not including too many noisy samples (i.e., those that are considered vulnerable but actually not) among the generated ones, without which the large scale would not be meaningful. 
With respect to the advances made by prior works and the challenges they face ($\S$\ref{sec:bkgmotive}), {\tech} achieves this goal in two phases. 

\vspace{3pt}\noindent
\ul{Phase 1: \textbf{Learning/training}}.
In this phase, {\tech} gets itself built up through two main tasks: (1) train a deep learning based model that can identify the code contexts in a given (normal) program where vulnerabilities can be injected and 
(2) mine vulnerability-introducing code edit patterns that can materialize the 
injection in the identified contexts. 
These two tasks are achieved in two steps, followed by preprocessing the datasets needed by this phase, as summarized below.

During \textbf{preprocessing}, {\tech} takes the \textit{source code} of given programs as input and performs \ul{value flow analysis} on them hence creates a graph representation of the resulting value flow information, referred to as their \textit{value flow graphs (VFGs)}. 
Then, two kinds of traversal paths are obtained from the VFG through \ul{sub-graph extraction}, resulting in two subgraphs, noted as \textit{relative and absolute VFG subgraphs}, respectively. 
These two subgraphs will be used %as sequences to learn 
to compute relative and absolute position encoding so as to enable our semantics-aware contextualization, and 
we choose value flow as the semantic information here as it is a precise form 
of data flow which has proven quite instrumental to recognizing vulnerable code~\cite{zhou2019devign}. 
Meanwhile, {\tech} computes the abstract syntax trees (\textit{ASTs}) of input programs via \ul{AST parsing}, followed by obtaining the \textit{linearized ASTs} via AST \ul{linearization} which are then concatenated with the corresponding source code's natural token sequence to form the \textit{Code+AST} input---this mixed/dual-format input is justified by its merits for learning the syntactic and contextual structures of code, especially via Transformer 
pre-training, as shown recently~\cite{niu2022spt}. Further details are in $\S$\ref{ssec:preprocessing}.

With these preprocessing capabilities, in its \textbf{Step 1: semantics-aware contextualization}, {\tech} first learns to 
contextualize vulnerability-injection code edits from existing vulnerability-introducing code locations retrieved (as discussed in $\S$\ref{sec:bkgmotive}) from a set of \textit{existing vulnerability fixes}. \modify{We use a set of vulnerability fixes rather than vulnerability introduction commits that originally introduced vulnerabilities, because mining vulnerability introduction commits in general is very difficult: (1) per a recent study~\cite{iannone2022secret}, most of the vulnerabilities are introduced from variable numbers of commits; (2) bug-introducing changes/commits are mostly not labeled because developers wouldn’t know that the changes introduce bugs at the time.}
To enable the semantics-awareness here, 
we designed a {\tt customized Transformer} that uses the \textit{Code+AST} format for its \ul{\tt input embedding} layer and computes \ul{\tt value-flow-based position encoding} in its self-attention blocks, as justified earlier ($\S$\ref{sec:bkgmotive}) and per the Transformer architecture.  
To actually gain this awareness as part of the general knowledge about 
code semantics as captured by the model, 
we leverage a large \textit{pre-training code corpus} (i.e., unlabeled data) by \ul{pre-training} the customized Transformer, as justified by the need 
to overcome the scarcity of our (labeled) {task-specific data} (i.e., the existing vulnerability-introducing code locations).  
Moreover, to make the general knowledge learned more transferable to our specific 
{downstream task} (i.e., vulnerability-injection code edit contextualization), 
we further introduce two new pre-training objectives, 
code-AST prediction ({\tt CAP}) \modify{which learns the information about the AST structure~\cite{niu2022spt}} and irrelevant statement prediction ({\tt ISP}) \modify{which learns identifying statements not impacting the main functionality of the program as they are more likely to inject vulnerabilities~\cite{nong2022generating}}, 
in addition to three existing general-purpose objectives~\cite{wang2021codet5}. 
{\tech} then trains the target contextualization model by \ul{fine-tuning} 
the pre-trained customized Transformer on the task-specific data (using the same preprocessing capabilities described above) for the downstream task. This step is elaborated in $\S$\ref{ssec:sac}.

Next, in \textbf{Step 2: human-knowledge-enhanced edit pattern formation}, 
{\tech} learns to materialize the code editing for realizing 
vulnerability injection from the concrete edits at the same vulnerability-introducing code locations mentioned above. 
To form such edit patterns, 
we first obtain the \textit{ASTs} of paired vulnerable and normal program samples 
retrieved from the existing vulnerability fixes (noted as ``seed samples")
via \ul{AST parsing}. 
To these paired ASTs, we apply an anti-unification 
%and hierarchical clustering 
based \ul{pattern extraction} algorithm~\cite{bader2019getafix}. 
However, the \textit{extracted patterns} are too many and many of them are too general or too specific to effectively guide vulnerability-injection code 
editing. 
We thus proceeded with \ul{pattern filtering and ranking} using a set of respective rules we defined. 
%
Importantly, to complement the seed samples' limited coverage of extant knowledge about vulnerability-introducing code edit patterns, 
we propose \ul{human knowledge discovery}---identifying additional patterns 
as well as mutation rules that may be applied to known patterns, both from \textit{vulnerability documentation} in the wild (CWE/CVEs and security bug reports). 
Next, we improved the generalizability of all the resulting patterns so far (including the \textit{filtered patterns} and \textit{manually defined patterns )}
via \ul{pattern refinement} (e.g., adding 
regex elements). %, which leads to the refined patterns. 
Lastly, applying the \textit{manually derived pattern mutation rules} to 
these \textit{refined patterns} leads us to the 
final set of \textit{vulnerability-injection code edit patterns}.
More details on this step are in $\S$\ref{ssec:hkeepf}.

\vspace{3pt}\noindent
\ul{Phase 2: \textbf{Production}}.
With the edit patterns and the 
{\tt trained contextualization model} both from the first phase, 
in this second phase {\tech} starts with \ul{preprocessing} (using the same module) a given set of \textit{normal programs} as input. 
Then, the model predicts all potential vulnerability-injection code edit 
contexts, where the editing is materialized as per the most suitable (for the contexts) edit pattern(s) through \ul{pattern matching and application}, 
resulting in the (expectedly) \textit{vulnerable samples} as 
elaborated in $\S$\ref{ssec:production}. 

% An overview of our {\tech} design is delineated in Figure~\ref{fig:overview}. At a high level, {\tech} works in two stages, \textit{learning} to generate vulnerability data  samples (at large scale) through \textit{injecting} vulnerable code into normal programs (in the wild). 
% In the \ul{learning} stage, {\tech} learns to 
% contextualize vulnerability-injection edits from 
% existing vulnerability-introducing code locations based on 
% a specialized deep code model. This model is pre-trained on a large code corpus against 3 
% existing general-purpose programming-language-oriented objectives and 2 new code-editing-specific objectives, followed by fine-tuning 
% Meanwhile, {\tech} learns to materialize the code editing for 
% vulnerability injection from the concrete edits at the same  vulnerability-introducing code locations. 
% The data required for these two learning steps are derived from an existing vulnerability-fixing dataset. 
% Then, in the \ul{injecting} stage, 
% {\tech} takes a normal program and transforms it to its vulnerable version by making vulnerability-injection 
% code changes (according to the learned vulnerability-introducing edit patterns) in the contexts predicted by 
% the learned contextualization model. 


==> overview.tex <==
\section{{\tech} Overview}
\cai{Overview is too long; I will work on the figure first and then have my version of overview in a different tex file}
\begin{figure*}[tp]
	\vspace{-0pt}
	\includegraphics[width=0.9\linewidth]{figures/overview.pdf}
	\caption{Overview of {\tech}.}
	\label{fig:overview}
	\vspace{-10pt}
\end{figure*}

Figure~\ref{fig:overview} shows an overview of {\tech}'s technical design. As shown, {\tech} consists of four main technical modules: preprocessing, localization learning, pattern mining, and vulnerability generation. To learn the high-quality vulnerability generation, {\tech} takes the existing vulnerability fixing data to train the vulnerability injection localization model and the vulnerability injection model, plus extra pre-training data to boost the performance of the localization model.
Given the training programs, {\tech} first preprocesses them into abstract syntax trees (ASTs), linearized ASTs for localization inputs, as well as relative and absolute value flow graph (VFG) sub-graphs. Then, the pattern mining module takes the ASTs to build the high-quality vulnerability injection patterns. The localization learning module takes the localization inputs and the relative and absolute VFG sub-graphs to learn a VGX-based Transformer model for vulnerability injection localization. Finally, given a normal program, the vulnerability generation module applies the trained vulnerability injection localization model and the vulnerability injection model which leverages the mined vulnerability injection patterns to generate high-quality vulnerable programs.

In the existing vulnerability fixing data, each sample is a pair of a vulnerable program and a respective fixed non-vulnerable (normal) program. The pre-training data is also pairs of programs which will be discussed in Section 4.1. Given pairs of programs, the preprocessing module uses an AST parser to convert them into pairs of ASTs for pattern mining. Since the localization model is in Transformer structure which takes text as the inputs, the preprocessing module applies AST linearization to convert the input ASTs into text, named linearized ASTs. The linearized ASTs are concatenated with the source code of the input program, and the concatenated text is the inputs for the VFG-based Transformer model. To improve the localization accuracy, the localization learning module also leverages the value flow graphs which contain semantic information of the programs for its self-attention blocks. Thus, the preprocessing module does a value flow analysis to get the value flow graphs (VFGs). Then, it extracts the relative and absolute VFG sub-graphs which will be fed into the self-attention blocks of the localization model. The details of the VFG and the sub-graph extraction will discussed in Section 4.2.

In the localization learning module, {\tech} trains a Transformer model for vulnerability injection localization. The model takes the concatenation of the source code and the linearized ASTs as the inputs. Next, it embeds the tokens in the inputs and feeds the embeddings to the encoders of the Transformer model. Then, the decoders of the Transformer model take the outputs of the encoders to generate new text. The Transformer model is trained to output the a statement to inject a vulnerability given a normal program. 

To improve the performance of the vulnerablity injection localization, we leverages a VFG-based position encoding in the self-attention blocks of the Transformer encoders as the VFG contains the semantic information of a program which is important for vulnerability injection localization. Specifically, a variable in a program should have higher attention to the variables which have value flows to it. Thus, for the variable tokens in the inputs, {\tech} extracts the VFG sub-graphs between the token and other variable tokens as we discussed in the preprocessing module, and uses the embeddings of these sub-graphs to compute the position encoding in the self-attention blocks to improve the understanding of the programs. 

Besides, pre-training is also widely proved to be helpful for understanding natural languages~\cite{devlin2018bert} and programming languages~\cite{feng2020codebert, wang2021codet5, niu2022spt}. Also, it allows to train a model without using very large training datasets, which is also the case in this work. Thus, to further improve the performance of the vulnerability injection localization model, we also leverages pre-training tasks for it. Based on our literature review, CodeT5~\cite{wang2021codet5} is one of the state-of-the-art pre-training model for code-to-code translation and the pre-training tasks are promising. Therefore, we first leverages the three pre-training tasks to improve the model understanding on the code. Then, since the model takes ASTs as part of the inputs and is specified for code localization, we built two other pre-training tasks. One is to build the connection between source code and the ASTs. The other one is to locate the statements that are irrelevant to the program functionalities.

In the pattern mining module, {\tech} takes the pairs of vulnerable and normal programs to mine a set of vulnerability injection patterns. It first takes the pairs of processed ASTs and extracts the differences between the ASTs. A difference is a pair of AST sub-trees which represents the code edits from the normal program to the vulnerable program, named concrete edits. Then, the pattern mining module applies the anti-unification and hierarchical clustering algorithms from Getafix~\cite{bader2019getafix} to build a set of edit patterns. However, the edit patterns are too many and many of them are too general or too specific to inject vulnerabilities. Thus, we build a set of filtering and ranking rules to get the edit patterns are suitable for vulnerability injection. We next manual adjust these edit patterns and add regular expression matching for some patterns to improve their generalizability. Finally, we mutate these patterns to further improve the generalizability and the patterns used to construct the vulnerability injection model.

With the trained vulnerability injection localization model and the vulnerability injection model, {\tech} can generate vulnerable programs given normal programs. In the vulnerability generation module, the vulnerability injection localization model predicts one or more candidate vulnerability injection locations given a normal program. Then, {\tech} applies the most suitable pattern(s) in the vulnerability injection model to the predicted candidate location(s). The program after the pattern application is expected to be vulnerable. 
